Measurements of $\phi_s$ at the LHCb experiment

These proceedings present the current status of measurements of the CP-violating phase $phi_s$ by the LHCb collaboration, reviewing the measurements in channels such as $B_s^0\to J/\psi\phi$, $B_s^0\to J/\psi \pi^+\pi^-$ and $B_s^0 \to \psi(2S)\phi$. The observation of the $B_s^0\to\eta_c\phi$ decay mode is presented for the first time, which can be used to measure $\phi_s$ with larger data samples that will be collected over the coming years by the LHCb experiment. Finally, the expected increase in precision from LHCb measurements of $\phi_s$ over the next decade is presented.

==> alias.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Newcommands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\comment}[1]{\par\noindent {\em\small [#1]}}
\renewcommand{\comment}[1]{}

% Subsection titles with text in math mode

\newcommand{\mysubsection}[1]{\subsection[#1]{\boldmath #1}}


% Units
\newcommand{\unit}[1]{\ensuremath{\rm\,#1}}
\newcommand{\keV}{\unit{keV}}
\newcommand{\keVc}{\unit{keV/{\it c}}}
\newcommand{\keVcc}{\unit{keV/{\it c}^2}}
\newcommand{\MeV}{\unit{MeV}}
\newcommand{\MeVc}{\unit{MeV\!/\!{\it c}}}
\newcommand{\MeVcc}{\unit{MeV\!/\!{\it c}^2}}
\newcommand{\MeVcca}{$\rm MeV\!/\!{\it c}^2$}
\newcommand{\GeV}{\unit{GeV}}
\newcommand{\GeVc}{\unit{GeV\!/\!{\it c}}}
\newcommand{\GeVcc}{\unit{GeV\!/\!{\it c}^2}}
\newcommand{\TeV}{\unit{TeV}}
\newcommand{\invfb}{\unit{fb^{-1}}}
\newcommand{\cm}{\unit{cm}}
\newcommand{\mm}{\unit{mm}}
\newcommand{\mb}{\unit{mb}}
\newcommand{\ps}{\unit{ps}}
\newcommand{\invps}{\unit{ps^{-1}}}
\newcommand{\invpsa}{$\rm ps^{-1}$}
\newcommand{\fs}{\unit{fs}}
\newcommand{\microns}{\unit{\mu m}}
\newcommand{\mrad}{\unit{mrad}}
\newcommand{\rad}{\unit{rad}}
\newcommand{\Hz}{\unit{Hz}}
\newcommand{\kHz}{\unit{kHz}}
\newcommand{\MHz}{\unit{MHz}}

% e.g. \ket{\Psi}=\sum_{i}\ket{\phi_i}\braket{\phi_i}{\Psi}

% Physics quantities

\newcommand{\CP}{\ensuremath{\rm CP}}
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}}


\newcommand{\IP}{\ensuremath{\rm IP}}
\newcommand{\signif}[1]{\ensuremath{\rm #1/\sigma_{#1}}}
\newcommand{\signifm}[1]{\ensuremath{#1/\sigma_{#1}}}
\newcommand{\pT}{\ensuremath{p_{\rm T}}}
\newcommand{\pTmin}{\ensuremath{\pT^{\rm min}}}
\newcommand{\ET}{\ensuremath{E_{\rm T}}}
\newcommand{\DLL}[2]{\ensuremath{\Delta  \ln{\cal L}_{\particle{#1}\particle{#2}}}}
\newcommand{\BR}[1]{\ensuremath{{\cal B} \rm (#1)}}
\newcommand{\BRvis}[1]{\ensuremath{{\cal B}_{\rm vis} \rm (#1)}}

\newcommand{\dm}{\ensuremath{\Delta m}}
\newcommand{\dms}{\ensuremath{\Delta m_{\rm s}}}
\newcommand{\dmd}{\ensuremath{\Delta m_{\rm d}}}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}}
\newcommand{\DGs}{\ensuremath{\Delta\Gamma_{\rm s}}}
\newcommand{\DGd}{\ensuremath{\Delta\Gamma_{\rm d}}}
\newcommand{\Gs}{\ensuremath{\Gamma_{\rm s}}}
\newcommand{\Gd}{\ensuremath{\Gamma_{\rm d}}}

\newcommand{\MBq}{\ensuremath{M_{\Bq}}}
\newcommand{\DGq}{\ensuremath{\Delta\Gamma_{\rm q}}}
\newcommand{\Gq}{\ensuremath{\Gamma_{\rm q}}}
\newcommand{\dmq}{\ensuremath{\Delta m_{\rm q}}}
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}}}
\newcommand{\GH}{\ensuremath{\Gamma_{\rm H}}}

\newcommand{\DGsGs}{\ensuremath{\Delta\Gamma_{\rm s}/\Gamma_{\rm s}}}
\newcommand{\Dm}{\mbox{$\Delta m $}}
\newcommand{\ACP}{\ensuremath{{\cal A}^{\rm CP}}}
\newcommand{\Adir}{\ensuremath{{\cal A}^{\rm dir}}}
\newcommand{\Amix}{\ensuremath{{\cal A}^{\rm mix}}}
\newcommand{\ADelta}{\ensuremath{{\cal A}^\Delta}}
\newcommand{\phid}{\ensuremath{\phi_{\rm d}}}
\newcommand{\sinphid}{\ensuremath{\sin\!\phid}}
\newcommand{\phis}{\ensuremath{\phi_{\rm s}}}
\newcommand{\betas}{\ensuremath{\beta_{\rm s}}}
\newcommand{\sbetas}{\ensuremath{\sigma(\beta_{\rm s})}}
\newcommand{\stbetas}{\ensuremath{\sigma(2\beta_{\rm s})}}
\newcommand{\stphis}{\ensuremath{\sigma(\phi_{\rm s})}}
\newcommand{\sinphis}{\ensuremath{\sin\!\phis}}


\newcommand{\vOmega}{\ensuremath{\vec{\Omega}}}
\newcommand{\vkappa}{\ensuremath{\vec{\kappa}}}
\newcommand{\vlambda}{\ensuremath{\vec{\lambda}}}

\newcommand{\Af}{\ensuremath{A_{f}}}
\newcommand{\Afbar}{\ensuremath{\overline{A}_{\overline{f}}}}
\newcommand{\fbar}{\ensuremath{\BAR{ f}}}

\newcommand{\calH}{\ensuremath{{\cal H}}}
% lifetime
\newcommand{\tauBs}{\ensuremath{\tau_\Bs}}
\newcommand{\tauL}{\ensuremath{\tau_{\rm L}}}
\newcommand{\tauH}{\ensuremath{\tau_{\rm H}}}



\newcommand{\effs}{{\ensuremath{\varepsilon^{\rm s}_\theta }}}
\newcommand{\effb}{{\ensuremath{\varepsilon^{\rm b}_\theta}}}


%CKM
\newcommand{\Vud}{\ensuremath{V_{\rm ud}}}
\newcommand{\Vus}{\ensuremath{V_{\rm us}}}
\newcommand{\Vub}{\ensuremath{V_{\rm ub}}}
\newcommand{\Vcd}{\ensuremath{V_{\rm cd}}}
\newcommand{\Vcs}{\ensuremath{V_{\rm cs}}}
\newcommand{\Vcb}{\ensuremath{V_{\rm cb}}}
\newcommand{\Vtd}{\ensuremath{V_{\rm td}}}
\newcommand{\Vts}{\ensuremath{V_{\rm ts}}}
\newcommand{\Vtb}{\ensuremath{V_{\rm tb}}}
\newcommand{\VCKM}{\ensuremath{V_{\rm CKM}}}

\newcommand{\Vjr}{\ensuremath{V_{ jr}}}
\newcommand{\Vjb}{\ensuremath{V_{j {\rm b}}}}




% tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\rm det}}}}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\rm rec/det}}}}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\rm sel/rec}}}}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\rm trg/sel}}}}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\rm tot}}}}

\newcommand{\mistag}{\ensuremath{\omega}}
\newcommand{\wcomb}{\ensuremath{\omega^{\rm comb}}}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\rm tag}}}}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\rm tag}^{\rm comb}}}}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\rm eff}}}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\rm eff}^{\rm comb}}}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}}
\newcommand{\effD}{{\ensuremath{\etag D^2}}}

\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\rm tag}^{\rm Pr}}}} %svecchi
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\rm tag}^{\rm LL}}}}

\newcommand{\tage}{\particle{e}}
\newcommand{\tagmu}{\particle{\mu}}
\newcommand{\tagKopp}{\particle{K_{opp}}}
\newcommand{\tagKsame}{\particle{K_{same}}}
\newcommand{\tagPsame}{\particle{\pi_{same}}}
\newcommand{\tagQvtx}{\ensuremath{Q_{\rm vtx}}}
\newcommand {\mch}      {\multicolumn {4} {|c|}}


% efficiencies
\newcommand{\effLO}{\ensuremath{\varepsilon_{\rm L0/sel}}}
\newcommand{\effpresel}{\ensuremath{\varepsilon_{\rm presel/gen}}}
\newcommand{\effsel}{\ensuremath{\varepsilon_{\rm sel/presel}}}
\newcommand{\effgen}{\ensuremath{\varepsilon_{\rm gen}}}


% Particle names

\newcommand{\BAR}[1]{\overline{#1}}

\newcommand{\particle}[1]{{\ensuremath{\rm #1}}}

\newcommand{\pp}{\particle{pp}}
\newcommand{\ppbar}{\particle{p\BAR{p}}}

\newcommand{\cc}{\particle{c\BAR{c}}}
\renewcommand{\b}{\particle{b}}
\newcommand{\bbar}{\particle{\BAR{b}}}
\newcommand{\bb}{\particle{b\BAR{b}}}
\newcommand{\dd}{\particle{d\BAR{d}}}

\newcommand{\B}{\particle{B}}
\newcommand{\Bd}{\particle{B^0}}
\newcommand{\Bs}{\particle{B^0_s}}
\newcommand{\Bds}{\particle{B^0_{(s)}}}
\newcommand{\Bu}{\particle{B^+}}
\newcommand{\Bc}{\particle{B^+_c}}
\newcommand{\Lb}{\particle{\Lambda_b}}

\newcommand{\Bbar}{\particle{\BAR{B}}}
\newcommand{\Bdbar}{\particle{\BAR{B}{^0}}}
\newcommand{\Bsbar}{\particle{\BAR{B}{^0_s}}}
\newcommand{\Bdsbar}{\particle{\BAR{B}{^0}_{(s)}}}
\newcommand{\Bubar}{\particle{B^-}}
\newcommand{\Bcbar}{\particle{B^-_c}}
\newcommand{\Lbbar}{\particle{\BAR{\Lambda}_b}}


\newcommand{\Bqq}{\particle{B_q}}
\newcommand{\Bqqbar}{\particle{\BAR{B_q}}}

\newcommand{\BL}{\particle{B_L}}
\newcommand{\BH}{\particle{B_H}}
\newcommand{\BLH}{\particle{B_{L,H}}}



\newcommand{\Ds}{\particle{D_s}}
\newcommand{\Dsm}{\particle{D_s^-}}
\newcommand{\KKpim}{\particle{K^+K^-\pi^-}}
\newcommand{\KK}{\particle{K^+K^-}}
\newcommand{\Dsp}{\particle{D_s^+}}
\newcommand{\Dsmp}{\particle{D_s^{\mp}}}

\newcommand{\Bq}{\particle{B_q}}
\newcommand{\Bqbar}{\particle{\BAR{B}_{q}}}

\newcommand{\Dz}{\particle{D^0}}
\newcommand{\Dzbar}{\particle{\BAR{D}{^0}}}
\newcommand{\DzCP}{\particle{D^0_{CP}}}
\newcommand{\Dstar}{\particle{D^{*-}}}
\newcommand{\Dstarz}{\particle{D^{0*}}}
\newcommand{\DstInc}{\particle{D^{(*)-}}}



\newcommand{\Jpsi}{\particle{J\!/\!\psi}}
\newcommand{\Jmm}{\particle{\Jpsi(\mu\mu)}}
\newcommand{\Jee}{\particle{\Jpsi(ee)}}
\newcommand{\ee}{\particle{e^+e^-}}
\newcommand{\JpsiX}{\particle{\Jpsi X}}

\newcommand{\KS}{\particle{K^0_S}}  
\newcommand{\Kst}{\particle{K^{*0}}}  
\newcommand{\Kstar}{\particle{K^{*}}}  
\newcommand{\Kstbar}{\particle{\BAR{K}^{*0}}}  

\newcommand{\Kplus}{\particle{K^+}}
\newcommand{\Kminus}{\particle{K^-}}
\newcommand{\Kpm}{\particle{K^\pm}}

\newcommand{\pip}{\particle{\pi^+}}
\newcommand{\pim}{\particle{\pi^-}}
\newcommand{\piz}{\particle{\pi^0}}

\newcommand{\Jphi}{\particle{J\!/\!\psi\phi}}
\newcommand{\BsBs}{\Bs--\Bsbar}
\newcommand{\BB}{\B--\Bbar}



% Decay channels

\newcommand{\decay}[2]{\particle{#1\!\to #2}}


\newcommand{\bccsbar}{\decay{\BAR{b}}{\BAR{c}c\BAR{s}}}

\newcommand{\KSpipi}{\decay{K^0_S}{\pi^+\pi^-}}  
\newcommand{\Jpsiee}{\decay{\Jpsi}{e^+e^-}}  
\newcommand{\Jpsimm}{\decay{\Jpsi}{\mu\mu}}  
\newcommand{\Jpsill}{\decay{\Jpsi}{\ell^+\ell^-}}  

\newcommand{\Kpi}{\particle{K^+\pi^-}}
\newcommand{\pippim}{\particle{\pi^+\pi^-}}


\newcommand{\DsKKpi}{\decay{\Dsm}{K^+K^-\pi^-}}  
\newcommand{\phiKK}{\decay{\phi}{K^+K^-}}
\newcommand{\KstKpi}{\decay{\Kst}{\Kpi}}


\newcommand{\Bdpipi}{\decay{\Bd}{\pi^+\pi^-}}            %  412100 Bd->pipi   
\newcommand{\BdKpi}{\decay{\Bd}{K^+\pi^-}}               %  412400 Bd->Kpi
\newcommand{\BspiK}{\decay{\Bs}{\pi^+K^-}}               %  612400 Bs->piK
\newcommand{\BsKK}{\decay{\Bs}{K^+K^-}}                  %  612500 Bs->KK
\newcommand{\Bhh}{\decay{\Bds}{h^+h^-}}                  %         B{d,s}->hh
\newcommand{\BsDspi}{\decay{\Bs}{\Dsm\pi^+}}             %  613350 Bs->Dspi
\newcommand{\BsDsK}{\decay{\Bs}{\Dsmp K^{\pm}}}          %  613450 Bs->DsK
\newcommand{\BsDsmKp}{\decay{\Bs}{\Dsm K^+}}             %  613450 Bs->DsK
\newcommand{\BsDspKm}{\decay{\Bs}{\Dsp K^-}}             %  613450 Bs->DsK
\newcommand{\BsDsh}{\decay{\Bs}{\Dsm h^+}}               %         Bs->Dsh
\newcommand{\BdJmmKS}{\decay{\Bd}{\Jmm\KS(\pi\pi)}}              %  411300 Bd->Jpsi(mumu)KS  
\newcommand{\BdJeeKS}{\decay{\Bd}{\Jee\KS}}              %  411400 Bd->Jpsi(mumu)KS  
\newcommand{\BdJKS}{\decay{\Bd}{\Jpsi\KS}}               %         Bd->JpsiKS  
\newcommand{\JKS}{\Jpsi\KS}
\newcommand{\BdbarJKS}{\decay{\Bdbar}{\Jpsi\KS}}

\newcommand{\BdJmmKst}{\decay{\Bd}{\Jmm\Kst(\particle{K}\pi)}}            %  411500 Bd->Jpsi(mumu)K*  
\newcommand{\BdJeeKst}{\decay{\Bd}{\Jee\Kst}}            %  411600 Bd->Jpsi(ee)K*  
\newcommand{\BdJKst}{\decay{\Bd}{\Jpsi\Kst}}             %         Bd->JpsiK*  
\newcommand{\BuJmmK}{\decay{\Bu}{\Jmm K^+}}              %         Bu->Jpsi(mumu)K  
\newcommand{\BuJeeK}{\decay{\Bu}{\Jee K^+}}              %         Bu->Jpsi(ee)K  
\newcommand{\BuJK}{\decay{\Bu}{\Jpsi K^+}}               %         Bu->JpsiK  

\newcommand{\BsDsmu}{\decay{\Bs}{\Dsm\mu^+\nu}}          %  Bs->Dsmunu


\newcommand{\BuJX}{\decay{\Bu}{\Jpsi X}}  
\newcommand{\BdJX}{\decay{\Bd}{\Jpsi X}}  
\newcommand{\BsJX}{\decay{\Bs}{\Jpsi X}}  
\newcommand{\LbJX}{\decay{\Lb}{\Jpsi X}}  
\newcommand{\BuJmmX}{\decay{\Bu}{\Jmm X}}  
\newcommand{\BdJmmX}{\decay{\Bd}{\Jmm X}}  
\newcommand{\BsJmmX}{\decay{\Bs}{\Jmm X}}  
\newcommand{\LbJmmX}{\decay{\Lb}{\Jmm X}}  
\newcommand{\bJX}{\decay{b}{\Jpsi X}}  
\newcommand{\BJX}{\decay{B}{\Jpsi X}}  

\newcommand{\BsJmmphi}{\decay{\Bs}{\Jmm\phi(\particle{KK})}}            %  611300 Bs->Jpsi(mumu)phi  
\newcommand{\BsJeephi}{\decay{\Bs}{\Jee\phi}}            %  611400 Bs->Jpsi(ee)phi  
\newcommand{\BsJeephiKK}{\decay{\Bs}{\Jee\phi(\particle{KK})}}            %  611400 Bs->Jpsi(ee)phi  
\newcommand{\BsJphi}{\decay{\Bs}{\Jpsi\phi}}             %         Bs->Jpsiphi  
\newcommand{\LbJL}{\decay{\Lambda_b}{\Jpsi\Lambda}}             %         Bs->Jpsiphi  
\newcommand{\Bsmm}{\decay{\Bs}{\mu^+\mu^-}}              %  612200 Bs->mumu  
\newcommand{\BdmmKst}{\decay{\Bd}{\mu^+\mu^-\Kst}}       %  411800 Bd->mumuK*  
\newcommand{\BdeeKst}{\decay{\Bd}{e^+e^-\Kst}}           %  411850 Bd->eeK*  
\newcommand{\BdllKst}{\decay{\Bd}{\ell^+\ell^-\Kst}}     %         Bd->llK*  
\newcommand{\BdphiKS}{\decay{\Bd}{\phi\KS}}              %  412000 Bd->phiKS
\newcommand{\Bsphiphi}{\decay{\Bs}{\phi\phi}}            %  615300 Bs->phiphi
\newcommand{\BsKstKst}{\decay{\Bs}{\Kst\Kst}}           
\newcommand{\BdDstpi}{\decay{\Bd}{D^{*-}\pi^+}}          %  415000 Bd->D*(excl)pi
\newcommand{\BdDstpiincl}{\decay{\Bd}{D^{*-}(incl)\pi^+}}%  415100 Bd->D*(incl)pi
\newcommand{\BdDKst}{\decay{\Bd}{\Dz\Kst}}               %         Bd->D0 K* 
\newcommand{\BdDbarKst}{\decay{\Bd}{\BAR{D}{^0}\Kst}}    %         Bd->D0~K* 
\newcommand{\BdDCPKst}{\decay{\Bd}{\DzCP\Kst}}           %         Bd->D0CP K* 
\newcommand{\BdDbarKpiKst}{\decay{\Bd}{\Dzbar(K\pi)\Kst}}%  414500 Bd->D0~(Kpi)K*
\newcommand{\BdDbarKKKst}{\decay{\Bd}{\Dzbar(KK)\Kst}}   %  414700 Bd->D0~(KK)K*
\newcommand{\BdDbarpipiKst}{\decay{\Bd}{\Dzbar(\pi\pi)\Kst}}   %  414800 Bd->D0~(pipi)K*
\newcommand{\BdDCPKKKst}{\decay{\Bd}{\DzCP(KK)\Kst}}   %         Bd->DCP(KK)K*
\newcommand{\BdKstrho}{\decay{\Bd}{K^{*0}\rho/\omega}}   %  418000 Bd->K*rho   
\newcommand{\Bsetacphi}{\decay{\Bs}{\eta_c\phi}}         %  615200 Bs->etacphi   
\newcommand{\BsetacKKphi}{\decay{\Bs}{\eta_c(4K)\phi}}   %         Bs->etac(4K)phi   
\newcommand{\BsetacpiKphi}{\decay{\Bs}{\eta_c(2pi2K)\phi}}  %         Bs->etac(2pi2K)phi   
\newcommand{\Bsetacpipiphi}{\decay{\Bs}{\eta_c(4pi)\phi}}%         Bs->etac(4pi)phi   
\newcommand{\BsJmmeta}{\decay{\Bs}{\Jmm\eta}}            %  611000 Bs->Jpsi(mumu)eta  
\newcommand{\BsJeeeta}{\decay{\Bs}{\Jee\eta}}            %  611200 Bs->Jpsi(ee)eta  
\newcommand{\BsJeta}{\decay{\Bs}{\Jpsi\eta}}             %         Bs->Jpsieta  
\newcommand{\BdKstgam}{\decay{\Bd}{K^{*0}\gamma}}        %  412500 Bd->K*gam  
\newcommand{\BdKstpin}{\decay{\Bd}{K^{*0}\pi^0}}         %  412700 Bd->K*pi0
\newcommand{\Bsphigam}{\decay{\Bs}{\phi\gamma}}          %  615000 Bs->phigam
\newcommand{\Bsphipin}{\decay{\Bs}{\phi\pi^0}}           %  ?????? Bs->phipi0
\newcommand{\Bdpipipi}{\decay{\Bd}{\pi^+\pi^-\pi^0}}     %  412800 Bd->3pi
\newcommand{\Bdrhopi}{\decay{\Bd}{\rho\pi}}              %  412800 Bd->3pi

\newcommand{\BcJmmpi}{\decay{\Bc}{\Jmm\pi^+}}            %  903000 Bc->Jpsi(mumu)pi  
\newcommand{\BcJpi}{\decay{\Bc}{\Jpsi\pi^+}}             %         Bc->Jpsi(mumu)pi  
\newcommand{\Bsmumu}{\decay{\Bs}{\mu^+\mu^-}}            %         Bs->mumu

\newcommand{\BsDsstDsst}{\decay{\Bs}{\Ds^{(*)-}\Ds^{(*)+}}}  
\newcommand{\BsDsDs}{\decay{\Bs}{\Dsm\Dsp}}             %  613350 Bs->Dspi
\newcommand{\BdDstmu}{\decay{\Bd}{\Dstar \mu^+\nu_\mu}}   %         

\newcommand{\BudsJX}{\decay{\rm B_{\rm u,d,s}}{\Jpsi \rm X}}


% text short cut

\newcommand{\SM}{Standard Model}             
\newcommand{\fsig}{\ensuremath{f_{\rm sig}}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}



% ADDED RECENTLY BY PELC

\newcommand{\mbs}{m_{\Bs}}   % Bs mass

\newcommand{\delone}{\delta_1}
\newcommand{\deltwo}{\delta_2}
\newcommand{\delperp}{\delta_{\perp}}
\newcommand{\delpar}{\delta_{\|}}
\newcommand{\delzero}{\delta_0}

%\def\thetaone{\theta_1}
\def\thetatwo{\theta_2}
\def\apar{A_{\|}(t)}
\def\aperp{A_{\perp}(t)}
\def\azero{A_{0}(t)}
\def\aparO{A_{\|}(0)}
\def\aperpO{A_{\perp}(0)}
\def\azeroO{A_{0}(0)}
\newcommand{\Rt}{R_\perp}
\newcommand{\Rp}{R_\|}
\newcommand{\Ro}{R_0}
\newcommand{\dGtwo}{\frac{\DG}{2}}
\renewcommand{\d}{{\rm d}}

\def\aparb{\bar{A}_{\|}(t)}
\def\aperpb{\bar{A}_{\perp}(t)}
\def\azerob{\bar{A}_{0}(t)}
\def\aparbO{\bar{A}_{\|}(0)}
\def\aperpbO{\bar{A}_{\perp}(0)}
\def\azerobO{\bar{A}_{0}(0)}


%OL: prefered notation for the angles:
%\def\thetatr{\theta}
%\def\phitr{\varphi}
%\def\thetaone{\psi}

\newcommand{\thetatr}{\ensuremath{\theta}}
\newcommand{\phitr}{\ensuremath{\varphi}}
\newcommand{\psitr}{\ensuremath{\psi}}
\newcommand{\thetaone}{\ensuremath{\psi}}



\newcommand{\phijphi}{\ensuremath{\phi_{\rm s}^{\Jphi}}}
\newcommand{\Phiphiphi}{\ensuremath{\Phi_{\Bsphiphi}}}
\newcommand{\myphis}{\ensuremath{\phi_{\rm s}}}

\newcommand{\phiM}{\ensuremath{\Phi_{\rm M}}}
\newcommand{\phiD}{\ensuremath{\Phi_{\rm D}}}
\newcommand{\phiCP}{\ensuremath{\Phi_{\rm CP}}}
\newcommand{\phiMNP}{\ensuremath{\Phi^{\rm NP}_{\rm M}}}
\newcommand{\phiDNP}{\ensuremath{\Phi^{\rm NP}_{\rm D}}}
\newcommand{\phiMG}{\ensuremath{\phi_{\rm s}^{\rm M/\Gamma}}}
\newcommand{\phiMGSM}{\ensuremath{\phi^{\rm M/\Gamma}_{\rm s \, ,SM}}}

\newcommand{\phipen}{\ensuremath{\Phi_{\rm penguin}}}
\newcommand{\phibox}{\ensuremath{\Phi_{\rm box}}}

\newcommand{\phiNP}{\ensuremath{\Phi^{\rm NP}}}
\newcommand{\phiSM}{\ensuremath{\phi_s^{\rm SM}}}
\newcommand{\phisDelta}{\ensuremath{\phi^\Delta_{\rm s}}}
\newcommand{\phitot}{\ensuremath{\Phi_{\rm tot}}}

\newcommand{\diffX}{ \frac{\d^{4} \Gamma}{\d t\, \d\Omega} }
\newcommand{\diffXbar}{ \frac{\d^{4} \bar \Gamma}{\d t\, \d\Omega} }

\newcommand{\calL}{\ensuremath{{\cal L}}}
\newcommand{\Ps}{\ensuremath{{\cal P}_{s}}}
\newcommand{\Psbar}{\ensuremath{\bar{{\cal P}_{s}}}}


==> preamble.tex <==
% THis file contains all the default packages and modifications for
% LHCb formatting

%% %%%%%%%%%%%%%%%%%%
%%  Page formatting
%% %%%%%%%%%%%%%%%%%%
%%\usepackage[margin=1in]{geometry}
\usepackage[top=1in, bottom=1.25in, left=1in, right=1in]{geometry}

% fallback for manual settings... uncomment if the geometry package is not available
%
%\voffset=-11mm
%\textheight=220mm
%\textwidth=160mm
%\oddsidemargin=0mm
%\evensidemargin=0mm

\columnsep=5mm
\addtolength{\belowcaptionskip}{0.5em}

\renewcommand{\textfraction}{0.01}
\renewcommand{\floatpagefraction}{0.99}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}

% Allow the page size to vary a bit ...
\raggedbottom
% To avoid Latex to be too fussy with line breaking ...
\sloppy

%% %%%%%%%%%%%%%%%%%%%%%%%
%% Packages to be used
%% %%%%%%%%%%%%%%%%%%%%%%% 
\usepackage{microtype}
\usepackage{lineno}  % for line numbering during review
\usepackage{xspace} % To avoid problems with missing or double spaces after
                    % predefined symbold
\usepackage{caption} %these three command get the figure and table captions automatically small
\renewcommand{\captionfont}{\small}
\renewcommand{\captionlabelfont}{\small}

%% Graphics
\usepackage{graphicx}  % to include figures (can also use other packages)
\usepackage{color}
\usepackage{colortbl}
\graphicspath{{./figs/}} % Make Latex search fig subdir for figures

%% Math
\usepackage{amsmath} % Adds a large collection of math symbols
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{upgreek} % Adds in support for greek letters in roman typeset

%% fix to allow peaceful coexistence of line numbering and
%% mathematical objects
%% http://www.latex-community.org/forum/viewtopic.php?f=5&t=163
%%
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
\expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
\expandafter\let\csname oldend#1\expandafter\endcsname\csname
end#1\endcsname
 \renewenvironment{#1}%
   {\linenomath\csname old#1\endcsname}%
   {\csname oldend#1\endcsname\endlinenomath}%
}
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}%
}
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
\patchBothAmsMathEnvironmentsForLineno{eqnarray}%
}

% Get hyperlinks to captions and in references.
% These do not work with revtex. Use "hypertext" as class option instead.
%\usepackage{hyperref}    % Hyperlinks in references
%\usepackage[all]{hypcap} % Internal hyperlinks to floats.

\input{lhcb-symbols-def} % Add in the predefined LHCb symbols

% Make this the last packages you include before the \begin{document}
\usepackage{cite} % Allows for ranges in citations
\usepackage{mciteplus}

